Balancing a CartPole System with Reinforcement Learning -- A Tutorial

In this paper, we provide the details of implementing various reinforcement learning (RL) algorithms for controlling a Cart-Pole system. In particular, we describe various RL concepts such as Q-learning, Deep Q Networks (DQN), Double DQN, Dueling networks, (prioritized) experience replay and show their effect on the learning performance. In the process, the readers will be introduced to OpenAI/Gym and Keras utilities used for implementing the above concepts. It is observed that DQN with PER provides best performance among all other architectures being able to solve the problem within 150 episodes.

==> pythoncode/pygtex <==
#! /usr/bin/env bash

## Write a .sty file defining the commands used in each Verbatim code block (bit hacky)
echo "" | pygmentize -l python -f latex -P full=True | head -n -10 | grep -E -v "documentclass|inputenc" > pygtex.sty

## Make a Verbatim code block for each input code file, transforming foo.ext to foo-ext.tex
for inname in $@; do
    outname=$(echo "$inname" | sed -e 's/[\ \.]/-/g').tex
    pygmentize -f latex -P verboptions='frame=leftline,framesep=1.5ex,framerule=0.8pt,fontsize=\tiny' $inname > $outname
done

